On Low-rank Trace Regression under General Sampling Distribution

In this paper, we study the trace regression when a matrix of parameters B* is estimated via the convex relaxation of a rank-regularized regression or via regularized non-convex optimization. It is known that these estimators satisfy near-optimal error bounds under assumptions on the rank, coherence, and spikiness of B*. We start by introducing a general notion of spikiness for B* that provides a generic recipe to prove the restricted strong convexity of the sampling operator of the trace regression and obtain near-optimal and non-asymptotic error bounds for the estimation error. Similar to the existing literature, these results require the regularization parameter to be above a certain theory-inspired threshold that depends on observation noise that may be unknown in practice. Next, we extend the error bounds to cases where the regularization parameter is chosen via cross-validation. This result is significant in that existing theoretical results on cross-validated estimators (Kale et al., 2011; Kumar et al., 2013; Abou-Moustafa and Szepesvari, 2017) do not apply to our setting since the estimators we study are not known to satisfy their required notion of stability. Finally, using simulations on synthetic and real data, we show that the cross-validated estimator selects a near-optimal penalty parameter and outperforms the theory-inspired approach of selecting the parameter.

==> estimator.tex <==
\section{RSS with nuclear norm penalty}
\label{sec:estimator}

By $\Loss:\IR^{d_r\times d_c}\to\IR^+\cup\{0\}$, we denote the sum-of-squares loss function with nuclear norm regularization, namely
\begin{align*}
\Loss(\bB):=\frac{1}{n}\norm{Y-\SamplingOp(\bB)}_2^2+\lambda\normNuc{\bB}.
\end{align*}
Let $\Sset\subseteq\IR^{d_r\times d_c}$ be a set of $d_r\times d_c$ matrices such that $\bBstar\in\Sset$. We will show that any $\Estimator$ that satisfies
\begin{align*}
\Loss(\Estimator)\leq\Loss(\bBstar)
\end{align*}
gives us an accurate estimate of $\bBstar$.


==> main-results.tex <==
\section{Estimators and Main Results}
\label{sec:trace-reg-nips}

This section contains our main results. We start by defining the family of estimators and the RSC condition. Then the general error bounds are presented in \S \ref{sec:trace-reg-nips}. \S \ref{sec:cross-val-brief-nips} contains our error bounds for the cross-validated estimator followed by its relevant simulations in \S \ref{sec:simulations}. Finally, \S \ref{subsec:applications-nips} contains applications of results of \S \ref{sec:trace-reg-nips} to the four classes of problems: matrix completion, multi-task learning, compressed sensing with Gaussian ensembles, and compressed sensing with factored measurements. A detailed version of this material with all the proofs is provided in the supplementary document.

\paragraph{General notions of rank and spikiness.} It is a well-known fact that, in Problem \ref{prob:main}, the low-rank assumption is not sufficient for estimating $\bBstar$ from the observations $Y$. For example, changing one entry of $\bBstar$ increases the rank of the matrix by (at most) 1 while it would be impossible to distinguish between these two cases unless the modified single entry is observed. To remedy this difficulty, \citet{candes2009exact,keshavan2009matrix} propose an incoherence assumption. If singular value decomposition (SVD) of $\bBstar$ is $\bU\bSigma\bV$, then the incoherence assumption roughly means that all rows of $\bU$ and $\bV$ have norms of the same order. Alternatively, \citet{negahban2012restricted} studied the problem under a different (and less restrictive) assumption, which bounds the \emph{spikiness} of the matrix $\bBstar$. Here, we define a general notion of spikiness and rank for a matrix that includes the one by \citet{negahban2012restricted} as a special case. We define \emph{spikiness} of a matrix $\bB\in\IR^{d_r\times d_c}$ by ${\SpikeNorm(\bB)}/{\normF{\bB}}$ and define its \emph{low-rankness} by ${\normNuc{\bB}}/{\normF{\bB}}$.

%
The spikiness used in \citet{negahban2012restricted} can be recovered by setting $\SpikeNorm(\bB)=\sqrt{d_rd_c}\norm{\bB}_\infty$. This choice of norm, however, is not suitable for many distributions for $\bX_i$'s. Two notable cases are multi-task learning and compressed sensing with factored measurements. In this paper, we show better choices for $\SpikeNorm(\cdot)$ for a given distribution.

Next, we state our assumptions and describe the estimation procedure.
%
\begin{assume}
\label{as:x-tilde-boundedness-deterministic-nips}
Assume that $\SpikeNorm(\bBstar)\leq \ParamBound$ for some $\ParamBound>0$.
\end{assume}
Note that in the above, we only require a bound on $\SpikeNorm(\bBstar)$ and \emph{not} the spikiness of $\bBstar$.

\begin{assume}
\label{as:gtmin-gtmax-bounds-nips}
For constants $\gmin,\gmax>0$, the following inequalities hold:
\[
\gmin\normF{\bB}^2
\leq
\norm{\bB}_{L^2(\SampleDistr)}^2
\leq
\gmax\normF{\bB}^2
\qquad\text{for all $\bB\in\IR^{d_r\times d_c}$}\,.
\]
\end{assume}
%
\begin{assume}
\label{as:x-tilde-boundedness-stochastic-nips}
There exists $\Cutoff>0$, such that $\IE{\inner{\bX,\bB}^2\cdot\II(\abs{\inner{\bX,\bB}}\leq\Cutoff)}\geq
\frac{1}{2}\IE{\inner{\bX,\bB}^2}$,
%
for all $\bB$ with $\SpikeNorm(\bB)\leq1$, where the expectations are with respect to $\SampleDistr$.
\end{assume}
%

\paragraph{Family of Estimators.} Our theoretical results enjoy a certain notion of algorithm independence. To make this point precise, we start by considering the following convex relaxation loss function, also stated in a different format in \eqref{eq:convex-opt-version-1},
%
\begin{align}
\Loss(\bB):=\frac{1}{n}\norm{Y-\SamplingOp(\bB)}_2^2+\lambda\normNuc{\bB}\,.\label{eq:main-loss-nips}
\end{align}
%
However, we do not necessarily need to find the global minimum of \eqref{eq:main-loss-nips}. Let $\Sset\subseteq\IR^{d_r\times d_c}$ be an arbitrary convex set of matrices with $\bBstar\in\Sset$. All of our bounds are stated for any \emph{any} $\Estimator$ that satisfies
%
\begin{align}
\label{eq:goodness-condition-nips}
\Estimator\in\Sset\quad\text{and}\quad\SpikeNorm(\Estimator)\leq \ParamBound\quad\text{and}\quad\Loss(\Estimator)\leq\Loss(\bBstar)\,.
\end{align}
%
While the global Minimizer, $\argmin_{\bB\in\Sset:\SpikeNorm(\bB)\leq b^*}\Loss(\bB)$, satisfies \eqref{eq:goodness-condition-nips}, we can also achieve this condition by using other loss minimization problems. A notable example would be to use the following non-convex optimization
%
\begin{align}
(\bUhat,\bVhat)=\argmin_{\bU\in\IR^{d_r\times r},\bV\in\IR^{d_c\times r}}\frac{1}{n}\norm{Y-\SamplingOp(\bU\bV^\top)}_2^2+\frac{\lambda}{2}\left(\normF{\bU}^2+\normF{\bV}^2\right)\,,
\label{eq:alt-min-loss-nips}
\end{align}
%
where $r$ is a pre-selected value for the rank. If we find the Minimizer of \eqref{eq:alt-min-loss-nips}, then it is known that $\Estimator=\bUhat\bVhat^\top$ satisfies \eqref{eq:goodness-condition-nips} (see  for example \cite{keshavan2009matrix} or \cite{mazumder2010spectral}).

%TBD: PLEASE ADD A REMARK ON INITIALIZING WITH NUCLEAR NORM WHEN PROBLEM CHANGES SLIGHTLY.

\subsection{Restricted Strong Convexity and the General Tail Bound} \label{subsec:bounds}

The upper bound that we will state relies on the \emph{restricted strong convexity} (RSC) condition.  For a \emph{constraint} set $\Cset\subseteq\IR^{d_r\times d_c}$, we say that $\SamplingOp(\cdot)$ satisfies RSC condition over $\Cset$ if there exists constants $\alpha(\SamplingOp)>0$ and $\beta(\SamplingOp)$ such that
\begin{align*}
\frac{1}{n}{\norm{\SamplingOp(\bB)}_2^2}\geq\alpha(\SamplingOp)\normF{\bB}^2-\beta(\SamplingOp)\,,
\end{align*}
for all $\bB\in\Cset$. In fact we work with a specific family of constraint sets that are parameterized by two positive numbers $\nu,\eta$, namely
%
\begin{align}
\Cset(\nu,\eta)
:=
\left\{
\bB\in\IR^{d_r\times d_c}
\given
\SpikeNorm(\bB)=1,~
\normF{\bB}^2\geq\nu,~
\normNuc{\bB}\leq\sqrt{\eta}\normF{\bB}
\right\}\,.\label{eq:Cset-def-nips}
\end{align}
%
We note that one can generalize the analysis of \cite{klopp2014noisy} and provide a deterministic upper bound for the estimation error (stated as Theorem \ref{thm:deterministic-error-bound} of \S \ref{sec:trace-reg} and proved in \S \ref{subsec:pf-thm-deterministic-error-bound} for completeness), when Assumption \ref{as:x-tilde-boundedness-deterministic-nips} holds, $\lambda\ge3\normOp{\bSigma}$, and the RSC condition holds for $\Cset(\nu,72r)$. Our next result shows that the RSC condition holds with high probability.
%
\begin{thm}[RSC]
\label{cor:rsc-condition-nips}
If Assumptions \ref{as:x-tilde-boundedness-deterministic-nips}-\ref{as:x-tilde-boundedness-stochastic-nips} hold, with probability greater than $1-2\exp\left(-\frac{Cn\gmin\nu}{\Cutoff^2}\right)$, the inequality
\begin{align}
\frac1n\norm{\SamplingOp(\bA)}_2^2\geq\frac\gmin4\normF{\bA}^2-\frac{93\eta\Cutoff^2}{\gmin}\IE{\normOp[\big]{\bSigma_R}}^2
\end{align}
holds for all $\bA\in\Cset(\nu,\eta)$, where $C>0$ is an absolute constant, provided that $Cn\gmin\nu>\Cutoff^2$.
\end{thm}
%
Theorem \ref{cor:rsc-condition-nips} is proved in \S \ref{sec:trace-reg} where it is denoted by Theorem \ref{cor:rsc-condition}.

Our main tail bound is the following corollary (stated also as Corollary \ref{cor:prob-trace-reg-error-bound} of \S \ref{sec:trace-reg} and proved there) which combines Theorem \ref{cor:rsc-condition-nips} and the general deterministic error bound (Theorem \ref{thm:deterministic-error-bound} of \S \ref{sec:trace-reg}) to obtain the following probabilistic error bound.
%
\begin{cor}
\label{cor:prob-trace-reg-error-bound-nips}
If Assumptions \ref{as:x-tilde-boundedness-deterministic-nips}-\ref{as:x-tilde-boundedness-stochastic-nips} hold, and let $\lambda\ge\lambda_1$ where $\lambda_1 := C\, \IE{\normOp[\big]{\bSigma_R}}\ParamBound\Cutoff$.
Then, under assumptions of Theorem \ref{thm:deterministic-error-bound} and Corollary \ref{cor:rsc-condition},
\begin{align*}
\normF[\big]{\Estimator-\bBstar}^2
&\leq
\frac{C'\lambda^2r}{\gmin^2},
\end{align*}
holds with probability at least $1-\IP{\lambda<3\normOp{\bSigma}}-\exp\left(-\frac{C''n\lambda^2r}{\Cutoff^2\ParamBound^2\gmin}\right)$ for constants $C, C', C''>0$.
\end{cor}
%
\begin{rem}[Optimality]\label{rem-optimality-nips} We will later show that Corollary \ref{cor:prob-trace-reg-error-bound} provides the same upper bound as in Corollary 1 of \citep{negahban2012restricted}, for the matrix completion problem, and as in Theorem 2.4 of \citep{candes2011tight}, for the compressed sensing case. In both of these papers the bounds are shown to be near optimal.
\end{rem}
\begin{rem}\label{rem-lambda-nips} While Corollary \ref{cor:prob-trace-reg-error-bound-nips} relies on two conditions for $\lambda$, namely $\lambda\ge \lambda_1$ and that $\IP{\lambda<3\normOp{\bSigma}}$ is small, only the latter condition is important to obtain a tail bound like \eqref{eq:trace-reg-bound} in Theorem \ref{thm:deterministic-error-bound} of \S \ref{sec:trace-reg}. The additional condition $\lambda\ge \lambda_1$ is only helping to make the upper bound simpler, i.e., ${C'\lambda^2r}/{\gmin^2}$ instead of the right hand side of \eqref{eq:trace-reg-bound}.
\end{rem}


\subsection{Tail Bound for the Cross-Validated Estimator}
\label{sec:cross-val-brief-nips}

In this section we obtain error bounds for a variant of the cross-validated estimator for our family of estimators $\Estimator$. Let $\{(\bX_i,y_i)\}_{i=1}^n$ be a set of observations and denote by $K$ the number of cross-validation folds. Let $\{\Iset_k\}_{k\in[K]}$ be a set of disjoint subsets of $[n]$ where $\cup_{k\in[K]}\Iset_k=[n]$. Letting $n_k:=\abs{\Iset_k}$, we have $n=n_1+\cdots+n_K$. Let $\SamplingOp_{k}(\cdot)$ and $\SamplingOp_{-k}(\cdot)$ be sampling operators for $\Iset_k$ and $[n]\setminus\Iset_{-k}$, respectively, and $Y_k$ and $Y_{-k}$ be the corresponding response vectors. In our analysis, we assume that the partition contains a large fraction of all samples, namely, we assume that $n_k\geq N/(2K)$ for all $k\in[K]$. Next, we assume that, for any $\lambda>0$, the estimators $\Estimator_{-k}(\lambda)$ satisfy \eqref{eq:goodness-condition-nips} for observations $(\SamplingOp_{-k}(\cdot),Y_{-k})$ for all $k\in[K]$. Define
$\ErrorCV(\lambda):=\sum_{k=1}^{K}\norm{Y_k-\SamplingOp_k(\Estimator_{-k}(\lambda))}_2^2$.
%
% glmnet: \cite{friedman2016lasso}
%Two methods for chosing $\widehat{\lambda}$ are discussed in \citep{friedman2010regularization}.

\begin{definition}\label{def:cvestimator-nips} Given a set $\Lambda=\{\lambda_1,\lambda_2,\cdots,\lambda_L\}$ of potential (positive) regularization parameters. Let $\PenaltyCV\in\arg\min_{\lambda\in\Lambda}\widehat{E}(\lambda)$, the $K$-fold cross-validated estimator with respect to $\Lambda$ is defined by
\begin{align*}
\EstimatorCV(\PenaltyCV):=\sum_{k=1}^{K}\frac{n_k}n\cdot\Estimator_{-k}(\PenaltyCV)\,.
\end{align*}
In the following we often use the more compact notation $\EstimatorCV$ instead of $\EstimatorCV(\PenaltyCV)$. We are now ready to state our error bound for $\EstimatorCV$.
\end{definition}
%
\begin{thm}
\label{cor:cv-estimator-explicit-bound-nips}
Let $\Lambda$, $\PenaltyCV$, and $\EstimatorCV$ be as in Definition \ref{def:cvestimator-nips}, and assume that $\lambda_0\in\Lambda$ satisfies conditions of Remark \ref{rem-lambda}. Assuming that $(\Noise_i)_{i=1}^n$ are independent mean-zero $\sigma_\Noise^2$-sub-Gaussian random variables, for all $t>0$, we have
\begin{align*}% nima
\normLTP[\big]{\EstimatorCV-\bBstar}^2
&\leq
\frac{C\gmax\lambda_0^2r}{\gmin^2}+2t,
\end{align*}
with probability at least
$1
-6KL\exp\left(-c\min\left(\frac{t^2}{\sigma_\Noise^4\vee\ParamBound^4},\frac{t}{\sigma_\Noise^2\vee\ParamBound^2}\right)\cdot\frac nK\right)
-\IP{\lambda_0\geq3\normOp{\bSigma}}-\exp\left(-\frac{C''n\lambda_0^2r}{\Cutoff^2\ParamBound^2\gmin}\right)
$.
\end{thm}
Theorem \ref{cor:cv-estimator-explicit-bound-nips} is stated as Corollary \ref{cor:cv-estimator-explicit-bound} of \S \ref{sec:cross-val} and is proved there.


\input{simulations}


\subsection{Applications}\label{subsec:applications-nips}

In this section, we will show the benefit of proving Corollary \ref{cor:prob-trace-reg-error-bound-nips} with a more general notion of spikiness. Specifically, we will look at four different special cases for the distribution $\SampleDistr$. In each case, the only things we need to compute are $\normLTP{\bB}$, $\norm{\bB}_{\psi_p(\SampleDistr)}$ for an appropriate $p$, and various constants. Two of these cases (matrix completion and compressed sensing with Gaussian ensembles) recover existing results by \cite{negahban2012restricted,klopp2014noisy} and \cite{candes2009exact} respectively. The other two, multi-task learning and compressed sensing with factored measurements, are (to the best of our knowledge) the first such results (e.g., stated as open problems in \cite{rohde2011estimation} and \cite{recht2010guaranteed} respectively). To simplify the notation, we assume $d_r=d_c=d$ throughout this section, however it is easy to see that the arguments hold for $d_r\neq d_c$ as well.
We also assume, for simplicity, that $\Noise_i\sim\Normal{0}{\sigma_\Noise^2}$ for all $i\in[n]$.

\paragraph{1) Matrix completion.} Let $\bBstar$ be a $d\times d$ matrix and recall that $e_1,e_2,\ldots,e_d$ denotes the standard basis for $\IR^d$. Let, also, for each $i\in[n]$, $r_i$ and $c_i$ be integers in $[d]$, selected independently and uniformly at random. Then,
let $\bX_i=\xi_i\cdot e_{r_i}e_{c_i}^\top$ where, for each $i$, $\xi_i$ is an independent
$4d^2$-sub-Gaussian random variable that is also independent of $r_j$ and $c_j$, $j\in[n]$. If we set $\xi_i:=d$ almost surely, then $\normSG{\xi_i}=d/\log2\leq2d$, and so, satisfies our requirement. This corresponds to the problem studied in \cite{negahban2012restricted}. One can alternatively use $\xi_i\sim\Normal{0}{4d^2}$. It, then, follows that
$\normLTP{\bB}=2\normF{\bB}$ and $
\normSGB{\bB}\leq 2d\normInf{\bB}$. We also set $\SpikeNorm(\cdot)=\normSGB{\cdot}$.
We can now use Lemma \ref{lem:freedman} (from \S \ref{subsec:bernstein}), for $\bZ_i:=\Noise_i\bX_i$ and $\nu:=d\sigma e/(e-1)$, to obtain bounds for $\IP{\lambda<3\normOp{\bSigma}}$ and $\IE{\normOp{\bSigma_R}}$, and apply Corollary \ref{cor:prob-trace-reg-error-bound-nips}, with $\ParamBound:=2d\normInf{\bBstar}$ and $\Cutoff:=9$, to obtain the following: when
$\lambda=C(\sigma_\Noise\vee\ParamBound)\sqrt{{\rho\,d}/n}$
for some $\rho\geq\log d$, we have that
%
\begin{align}
\label{eq:mc-error-bound-nips}
\normF[\big]{\Estimator-\bBstar}^2
&\leq
C'(\sigma_\Noise^2\vee\ParamBound^2)\:\frac{\rho\,dr}{n},
\end{align}
%
with probability at least $1-\exp(-C''\rho)$, which resembles Corollary 1 in \cite{negahban2012restricted} with $\rho=\log d$. Details of the above stNoise is provided in \S \ref{subsec:matrix-completion}.

\paragraph{2) Multi-task learning.} Similar as in the matrix completion case, let $\bBstar$ be a $d\times d$ matrix and
let for each $i\in[n]$, $r_i$ be an integer in $[n]$, selected independently and uniformly at random. Then let $\bX_i=e_{r_i}\cdot X_i^\top$ where, for each $i$, $X_i$ is an independent $\Normal{0}{d\cdot\Eye_d}$ random vector that is also independent of $r_j$, $j\in[n]$. It then follows that $\normLTP{\bB}=\normF{\bB}$. Then
and
$\normSGB{\bB}\leq\sqrt{d}\norm{\bB}_{\infty,2}$. We also set $\SpikeNorm(\cdot)=\normSGB{\cdot}$. Now we can apply Lemma \ref{lem:freedman} with the same  $\bZ_i$ and $\nu$ as above. It is also easy to verify that $\gmin=1$ and $\Cutoff=9$ meets the requirements for these parameters, and so, by taking any $\ParamBound\geq\sqrt{d}\norm{\bBstar}_{\infty,2}$, we conclude that \eqref{eq:mc-error-bound-nips} holds in this case as well, with the same probability. Details of these stNoise is provided in \S \ref{subsec:bandit-regression}.

\paragraph{3) Compressed sensing via Gaussian ensembles.} Let $\bBstar$ be a $d\times d$ matrix.
Let each $\bX_i$ be a random matrix with entries filled with i.i.d. samples drawn from $\Normal{0}{1}$. It then follows that $\normLTP{\bB}=\normF{\bB}$ and $\normSGB{\bB}=\normF{\bB}$. We also set $\SpikeNorm(\cdot)=\normSGB{\cdot}$.
%
An argument similar to that of multi-task learning proves that \eqref{eq:mc-error-bound-nips} holds for this setting with $\ParamBound\geq\normF{\bBstar}$. This bound resembles the bound of \cite{candes2011tight}.

\paragraph{4) Compressed sensing via factored measurements.} \citet{recht2010guaranteed} propose factored measurements to alleviate the need to a storage of size $nd^2$ for compressed sensing applications with large dimensions. The idea is to make measurements of the form $UV^\top$ where $U$ and $V$ are random vector of length $d$. Even though $UV^\top$ is still a $d\times d$ matrix, but, we only need a memory of size $\Order{nd}$ to store all the input, which is a huge improvement compared to Gaussian ensembles. Now, we study this problem when $U$ and $V$ are both $\Normal{0}{\Eye_d}$ vectors that are independent of each other. We can then show (after a long derivation that is given in \S \ref{subsec:factored-meas}) that $\normLTP{\bB} =\normF{\bB}^2$ and $\norm{\bB}_{\psi_1(\SampleDistr)}\leq
({8}/{\sqrt{\log 2}})\normF{\bB}$. Now, setting $\SpikeNorm(\cdot)=\norm{\cdot}_{\psi_1(\SampleDistr)}$, the same bound as \eqref{eq:mc-error-bound-nips} works with slightly different constants.

